Performance Evaluation of Mixed-Precision Runge-Kutta Methods

Additive Runge-Kutta methods designed for preserving highly accurate solutions in mixed-precision computation were proposed and analyzed in [8]. These specially designed methods use reduced precision or the implicit computations and full precision for the explicit computations. We develop a FORTRAN code to solve a nonlinear system of ordinary differential equations using the mixed precision additive Runge-Kutta (MP-ARK) methods on IBM POWER9 and Intel x86\_64 chips. The convergence, accuracy, runtime, and energy consumption of these methods is explored. We show that these MP-ARK methods efficiently produce accurate solutions with significant reductions in runtime (and by extension energy consumption).

==> tables.tex <==
\begin{tabular}{ |c|c|c|c|c|c|  }
 \hline
 \multicolumn{6}{|c|}{IM-1p Runtime (s) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.000711 & 0.000127 & 0.000068& 0.000114& 0.000066& 0.000066\\
 0.005860 & 0.000494 & 0.000268& 0.000438& 0.000180& 0.000173\\
 0.029061 & 0.003237 & 0.001754& 0.002614& 0.000938& 0.000974\\
 0.200017 & 0.018010 & 0.010076& 0.012969& 0.004921& 0.004857\\
 \hline
 \multicolumn{6}{|c|}{SDIRK-3p Runtime (s) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.001312 & 0.000154 & 0.000106 & 0.000104 & 0.000061 & 0.000062\\
 0.005928 & 0.000849 & 0.000656 & 0.000445 & 0.000224 & 0.000246\\
 0.031965 & 0.005722 & 0.004847 & 0.003261 & 0.002162 & 0.002074\\
 0.253049 & 0.045016 & 0.031873 & 0.018709 & 0.009515 & 0.009710\\
 \hline
 \multicolumn{6}{|c|}{Novel Method 4s3pA Runtime (s) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.001543 & 0.000273 & 0.000194& 0.000199& 0.000134& 0.000136\\
 0.011115 & 0.001399 & 0.000811& 0.000915& 0.000340& 0.000378\\
 0.062933 & 0.007696 & 0.005559& 0.004917& 0.002095& 0.002157\\
 0.430059 & 0.052646 & 0.035969& 0.026183& 0.009849& 0.009585\\
 \hline
\end{tabular}

\begin{tabular}{ |c|c|c|c|c|c|  }
 \hline
 \multicolumn{6}{|c|}{IM-1p Energy Consumption (Joules) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.049744 & 0.036462 & 0.044959 & 0.050281 & 0.036926 & 0.032813\\
 0.159118 & 0.050097 & 0.049841 & 0.045911 & 0.035938 & 0.036951\\
 0.910398 & 0.094299 & 0.070422 & 0.078406 & 0.057129 & 0.053747\\
 6.473018 & 0.577672 & 0.310851 & 0.427819 & 0.153808 & 0.148559\\
 \hline
 \multicolumn{6}{|c|}{SDIRK-3p Energy Consumption (Joules) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.071838 & 0.046496 & 0.039599 & 0.047351 & 0.034021 & 0.038892\\
 0.165441 & 0.051184 & 0.051196 & 0.041333 & 0.054175 & 0.051135\\
 1.022189 & 0.162341 & 0.136706 & 0.091602 & 0.083764 & 0.075671\\
 8.298050 & 1.292672 & 1.028257 & 0.608995 & 0.282971 & 0.297912\\
 \hline
 \multicolumn{6}{|c|}{Novel Method 4s3pA Energy Consumption (Joules) for x86} \\
 \hline
 real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
 \hline
 0.064453 & 0.042297 & 0.047803 & 0.038269 & 0.048828 & 0.039978\\
 0.327233 & 0.070776 & 0.057043 & 0.066992 & 0.042712 & 0.043274\\
 2.083210 & 0.217529 & 0.153747 & 0.131237 & 0.072473 & 0.074780\\
 14.091297 & 1.713252 & 1.131870 & 0.859373 & 0.297594 & 0.285473\\
 \hline
\end{tabular}

%\begin{tabular}{ |c|c|c|c|c|c|  }
% \hline
%\multicolumn{6}{|c|}{IM-1p Runtime (s) for Power9} \\
% \hline
% real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
% \hline
% 0.000160 & 0.000123 & 0.000067& 0.000123& 0.000069& 0.000068\\
% 0.001475 & 0.000521 & 0.000214& 0.000509& 0.000206& 0.000211\\
% 0.010053 & 0.003126 & 0.001250& 0.003063& 0.001201& 0.001211\\
% 0.073585 & 0.022139 & 0.007639& 0.021594& 0.007134& 0.007334\\
% \hline
% \multicolumn{6}{|c|}{SDIRK-3p Runtime (s) for Power9} \\
% \hline
% real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
% \hline
% 0.000289 & 0.000118 & 0.000068& 0.000128& 0.000061& 0.000060\\
% 0.001474 & 0.000617 & 0.000333& 0.000589& 0.000308& 0.000308\\
% 0.010242 & 0.004347 & 0.002977& 0.004053& 0.002709& 0.002718\\
% 0.092578 & 0.034395 & 0.019270& 0.031540& 0.016639& 0.017124\\
% \hline
% \multicolumn{6}{|c|}{Novel Method 4s3pA Runtime (s) for Power9} \\
% \hline
% real128,real128 & real128,real64 & real128,real32 & real64,real64 & real64,real32 & real32,real32\\
% \hline
% 0.000321 & 0.000291 & 0.000163& 0.000248& 0.000161& 0.000163\\
% 0.003142 & 0.001245 & 0.000482& 0.001132& 0.000475& 0.000479\\
% 0.020565 & 0.006853 & 0.002965& 0.007067& 0.002869& 0.002930\\
% 0.140042 & 0.049135 & 0.018296& 0.047340& 0.017068& 0.017110\\
% \hline
%\end{tabular}
